InferCode: Self-Supervised Learning of Code Representations by Predicting Subtrees

Building deep learning models on source code has found many successful software engineering applications, such as code search, code comment generation, bug detection, code migration, and so on. Current learning techniques, however, have a major drawback that these models are mostly trained on datasets labeled for particular downstream tasks, and code representations may not be suitable for other tasks. While some techniques produce representations from unlabeled code, they are far from satisfactory when applied to downstream tasks. Although certain techniques generate representations from unlabeled code when applied to downstream tasks they are far from satisfactory. This paper proposes InferCode to overcome the limitation by adapting the self-supervised learning mechanism to build source code model. The key novelty lies in training code representations by predicting automatically identified subtrees from the context of the ASTs. Subtrees in ASTs are treated with InferCode as the labels for training code representations without any human labeling effort or the overhead of expensive graph construction, and the trained representations are no longer tied to any specific downstream tasks or code units. We trained an InferCode model instance using the Tree-based CNN as the encoder of a large set of Java code and applied it to downstream unsupervised tasks such as code clustering, code clone detection, cross-language code search or reused under a transfer learning scheme to continue training the model weights for supervised tasks such as code classification and method name prediction. Compared to previous code learning techniques applied to the same downstream tasks, such as Code2Vec, Code2Seq, ASTNN, higher performance results are achieved using our pre-trained InferCode model with a significant margin for most tasks including those involving different programming languages.

==> details.tex <==
%!TEX root=main.tex
\subsection{Proposed approach}

Because the conventional neural network for source code modeling lacks of the interpretability purpose, we introduce the attention mechanism to both the GGNN and TBCNN for the interpretability purpose. There are two key intuitions:

- The attention mechanism will assign a score to each of the node in the AST tree; and the scores indicate the importance of the node for the task.

- To find the important code components is to delete them from the original code and measure how the deletion affects on the  predicted probability, i.e the difference between the confidence score of the correct class between the original program and the changed program. We call this difference as "delta". From our empirical evaluation, we found that there are a strong correlation between the delta and the attention score, as we will show later in Section.

Figure ~\ref{figure:overview}  shows the overview of our approach. 

From a non-interpretable neural network, we introduce the attention mechanism as the aggregation layer as a better way to combine the nodes to make the neural network becomes interpretable. (1) From a test program, we put it into the Attention NN to produce the attention scores (2) and the confidence score (3) of the correct class of the program. We also introduce a perturbation engine to delete the code components one by one. We use the same test program as the input of the perturbation engine (4). Once the program has been perturbed (5), we repeat the same 

\begin{figure}[h]
	\centering
	\includegraphics[width=1.0\columnwidth]{figs/overview.png}
	\caption{Overview of our approach}
	\label{figure:overview}
\end{figure}


We proposed an approach to modify the aggregation layer of TBCNN, which takes the inspiration from GGNN. In Figure \ref{figure:proposed_approach}, since we have the node representation matrix, we feed the matrix into 2 different blocks, the first block is the attention network, which is a feed forward network with non-linearity at the output that squeezes dimension 0 of the matrix into 1-dimension transpose vector where each vector represents how much a node contributes the objective. The second block is simply a dynamic pooling block that takes the max of each feature,  which is the dimension 1 of the matrix into a feature vector that represents for structure-level. 

Supposed that we have an M X N feature matrix, from the attention network, we can get the M X 1 vector that score how much each node has contributed, and from the dynamic pooling block, we can get the 1 X N vector that represents for structure-level, which is also useful to represent how the feature vector is changed for different type of input. 

Once we get the 2 output, we multiply these 2 outputs and form a feature matrix again, then apply the dynamic pooling on this feature to get one final feature vectors for the structure-level representation. Thus this end-to-end process represents for the Aggregation block in Figure \ref{figure:general} to enable the explainability for the TBCNN.

Figure~\ref{figure:sample_coloring} shows an example of how attention network can help to visualize contribution of nodes, either for GGNN or TBCNN. Since the score of each node is range from 0-1 if we choose the sigmoid function for non-linearity, the darkness level of the color of a node increase when the score is increased and vice versa. 

Moreover, with the attention layer, one can visualize the learning process through back-propagation. In neural network training, errors are backpropagated from output layers to each intermediate layer and finally to the original inputs, the attention layer, in this case, can act as the observer to monitor how the features are extracted through the learning process.

\lx{adding the attention layer may indeed improve the scoring of the nodes and improve the visualization, but is it necessary for visualization? Even without the attention layer, TBCNN and GGNN should have already trained some scores/weights for the nodes; what are those weights look like when visualized?}

